Communication-Critical Planning via Multi-Agent Trajectory Exchange

This paper addresses the task of joint multi-agent perception and planning, especially as it relates to the real-world challenge of collision-free navigation for connected self-driving vehicles. For this task, several communication-enabled vehicles must navigate through a busy intersection while avoiding collisions with each other and with obstacles. To this end, this paper proposes a learnable costmap-based planning mechanism, given raw perceptual data, that is (1) distributed, (2) uncertainty-aware, and (3) bandwidth-efficient. Our method produces a costmap and uncertainty-aware entropy map to sort and fuse candidate trajectories as evaluated across multiple-agents. The proposed method demonstrates several favorable performance trends on a suite of open-source overhead datasets as well as within a novel communication-critical simulator. It produces accurate semantic occupancy forecasts as an intermediate perception output, attaining a 72.5% average pixel-wise classification accuracy. By selecting the top trajectory, the multi-agent method scales well with the number of agents, reducing the hard collision rate by up to 57% with eight agents compared to the single-agent version.

==> figure/datasetranks.tex <==
\begin{figure*}
\vspace{2mm}
\centering
\includegraphics[width=0.8\linewidth]{./figure/datasetranks.png}
\caption{\textbf{Trajectory Rank versus Collision Rate}.  Prioritized trajectories for the \textbf{BlindCorner}, \textbf{AutoCastSim-RedLight}, and \textbf{CrissCross} dataset scenarios, respectively.}
\label{fig:datasetranks}%
\end{figure*} 

